Cooperative Training and Latent Space Data Augmentation for Robust Medical Image Segmentation

Deep learning-based segmentation methods are vulnerable to unforeseen data distribution shifts during deployment, e.g. change of image appearances or contrasts caused by different scanners, unexpected imaging artifacts etc. In this paper, we present a cooperative framework for training image segmentation models and a latent space augmentation method for generating hard examples. Both contributions improve model generalization and robustness with limited data. The cooperative training framework consists of a fast-thinking network (FTN) and a slow-thinking network (STN). The FTN learns decoupled image features and shape features for image reconstruction and segmentation tasks. The STN learns shape priors for segmentation correction and refinement. The two networks are trained in a cooperative manner. The latent space augmentation generates challenging examples for training by masking the decoupled latent space in both channel-wise and spatial-wise manners. We performed extensive experiments on public cardiac imaging datasets. Using only 10 subjects from a single site for training, we demonstrated improved cross-site segmentation performance and increased robustness against various unforeseen imaging artifacts compared to strong baseline methods. Particularly, cooperative training with latent space data augmentation yields 15% improvement in terms of average Dice score when compared to a standard training method.

==> figures/hard_example.tex <==
% \setlength\intextsep{0pt}
% %% combine table and figure together:
% \begin{table}%
% \centering
% \parbox{0.2\textwidth}{
% \begin{footnotesize}
% \centering
% \caption{Effectiveness of targeted masking, latent code filtering and joint training}
% \label{tab:ablation_joint_training_and_code_filteting}
% \begin{adjustbox}{width=0.2\textwidth}
% \begin{tabular}{@{}c|cc@{}}
% \toprule
% Methods & \FTN & \FTN+\STN \\ \midrule
% w.o. $\gch,\gsp$ &  0.6344 & 0.6584 \\ \midrule
% % UNet~\cite{Ronneberger_2015_unet}& 0.6396 & -\\
% share code (a) ($\zi=\zi, \zs = \zi$) & 0.6625 & 0. 6868  \\
% share code (b)  $(\zi=\zs, \zs=\zs)$ & {0.6343} & {0.6587} \\ \midrule
% Separate Training~\cite{Larrazabal_2019_MICCAI_DAE}  & 0.6020 & 0.6077 \\ \midrule
% The proposed & \textbf{0.6711} & \textbf{0.6901} \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{footnotesize}
% }
% \qquad
% \begin{minipage}[c]{0.7\textwidth}%
% \centering
% \includegraphics[width=0.7\textwidth]{images/hard_examples.png}
% \captionof{figure}{Visualization of generated hard examples with the proposed three mask schemes. For targeted code masking, we set $w$=0 for ease of comparison.}
% \label{fig:hard_example}
% \end{minipage}
% \end{table}
% \setlength\intextsep{0pt}
\setlength\intextsep{0pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/hard_examples.png}
    \caption{{Visualization of generated hard examples with the three masking schemes ($a$=0 for ease of comparison). Best viewed in zoom-in.}}
    \label{fig:hard_example}
\end{figure}
\setlength\intextsep{0pt}


==> figures/introduction_figure.tex <==
\setlength\intextsep{0pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/overview.png}
    \caption{(a) The proposed cooperative training framework, which consists of a fast-thinking network (\FTN) and a slow-thinking network (\STN).
    % \FTN\ employs an encoder $\Ei$ and a latent code filter $\filter$ to map images $\image$ or corrupted images $\hat\image$ to two latent codes: a image-related code $\zi$ which carries image contextual information and a shape-related code $\zs$ which carries task-related object shape information. These codes are then projected back to image and segmentation space using decoders $\Di$ and $\Ds$. \STN\ is denoising autoencoder $\C$, which is used to refine the network prediction $\prediction$ and/or corrupted prediction $\hat\prediction$. 
    (b) Hard example generation in latent space. Latent code masking is performed for generating both corrupted images and segmentations for cooperative training.}
    % The corrupted images and segmentation $\hat\image,\hat\prediction$ are automatically generated by \FTN\ via latent code masking. These hard examples are used to assist the training of both networks. Code masks $\mask$ are generated in either random or adversarial targeted fashion. 
    % Please refer to Sec.\ref{SEC:latent_code_masking} for more details.}
    \label{fig:introduction}
\end{figure}
\setlength\intextsep{0pt}


==> figures/standard_vs_cooperative.tex <==
\setlength\intextsep{0pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/standard_vs_cooperative.png}
    \caption{Compared to standard training, cooperative training with self-generating hard examples greatly improves the segmentation performance on various \emph{unseen, challenging} domains (p-value$<0.01$, average improvement: 15\%).}
    \label{fig:standard_vs_cooperative}
\end{figure}
\setlength\intextsep{0pt}

